A-NICE-MC: Adversarial Training for MCMC

Existing Markov Chain Monte Carlo (MCMC) methods are either based on general-purpose and domain-agnostic schemes which can lead to slow convergence, or hand-crafting of problem-specific proposals by an expert. We propose A-NICE-MC, a novel method to train flexible parametric Markov chain kernels to produce samples with desired properties. First, we propose an efficient likelihood-free adversarial training method to train a Markov chain and mimic a given data distribution. Then, we leverage flexible volume preserving flows to obtain parametric kernels for MCMC. Using a bootstrap approach, we show how to train efficient Markov chains to sample from a prescribed posterior distribution by iteratively improving the quality of both the model and the samples. A-NICE-MC provides the first framework to automatically design efficient domain-specific MCMC proposals. Empirical results demonstrate that A-NICE-MC combines the strong guarantees of MCMC with the expressiveness of deep neural networks, and is able to significantly outperform competing methods such as Hamiltonian Monte Carlo.

==> backup.tex <==
Let $\mc{S}$ be the state space for the sequence of random variables $\mc{X} = \{\Xv_t\}_{t=0}^{t=\infty}$, $\Xv_t \in \mc{S}$. Let $\pi^0$ be an initial probability distribution for $\Xv_0$, and $T_\theta(\cdot|\xv)$ be a transition kernel parameterized by $\theta$, e.g., using a neural network.
We assume $T_\theta$ is easy to sample from, and is a valid transition kernel for any choice of $\theta$, i.e., it satisfies 
$\int_{\mc{S}} T_\theta(\xv'|\xv) \text{d}\xv' = 1$ for all $\xv \in \mc{S}$. 
Therefore, every $T_\theta$ defines a time-homogeneous Markov chain over $\mc{X}$. We denote $\pi^t_\theta(\xv)$ the resulting probability distribution at time step $t$.
If we assume that $T_\theta(\xv_t|\xv_{t-1}) > 0$ for all $\xv_t, \xv_{t-1} \in \mc{S}$, then the Markov chain defined by $T_\theta$ is both irreducible and positive recurrent, and hence has a unique stationary distribution $\pi_\theta = \Lim{t \rightarrow \infty} \pi^t_\theta$. 
For all $\xv \in \mc{S}$, $\pi_\theta$ satisfies 
\begin{equation}
\pi_\theta(\xv) = \int_\mc{S} T_\theta(\xv|\xv') \pi_\theta(\xv') \text{d}\xv' \label{eq:stationary}
\end{equation}

Suppose there is an unknown distribution $p_d(\xv)$ from which we can obtain samples from, e.g., a data distribution. Our goal here is twofold: we want to find a $\theta$ such that 1) $\pi_\theta$ is close to $p_d(\xv)$, and 2) the corresponding Markov Chain mixes quickly.


% \section{Analytic target}
% \js{maybe define "model" and "proposal" in the problem setup? In the data case, "proposal" is "model", in the mcmc case, "proposal" is not exactly "model", but "forward-backward" like}

% Suppose $p_d$ is given by an analytic expression, known up to normalization constant. typical case: posterior in bayesian inference, graphics, scientific computing. two challenges: we don't have access to samples from $p_d$, and want to set up a markov chain where $\pi_\theta$ (the underlying limiting distribution) is \emph{exactly} $p_d$.

% \subsection{exact sampling}
% idea: restrict possible kernels to ones satisfying detailed balance with respect to $p_d$. define a proposal, then correct it with metropolis-hastings.

% discuss reinforce option

% discuss flow option, hmc

% problem: residual connection in NICE to make Jacobian det 1.

% options: scale inputs 

% \subsection{pairwise discriminator for decreased autocorrelation}
% \js{pairwise discriminator works for models even with residual connections}


% \subsection{bootstrap}
% challenge: we don't have access to samples $p_d$ for our gan style approach. the idea is to bootstrap the process. we start from a valid (but possibly slow mixing) markov chain $T_{\theta_0}$ with stationary distribution $p_d$, and an arbitrary initial distribution $\pi^0$. we produce samples from $\pi^{k_0}_{\theta_0}$ (running the chain for $k_0$ steps), and using these samples we train a new chain $T_{\theta_1}$ such that $\pi^{k_0}_{\theta_0} \approx \pi^{k_1}_{\theta_1}$ with $k_1 \ll k_0$. repeat the process.
% \js{This is not done exactly like this; also \cite{li2017approximate} has a similar idea (of ``distilling'' a markov chain, so I wonder if the reviewers would doubt the novelty if we describe in this way}

% \subsubsection{new loss on real datasets}
% Figures to show that new discriminator loss will help mixing
% \js{Our new objective allows us to directly train for better ESS}

% \section{Experiments}

% \subsection{Learning from data}
% iclr experiments
% \js{I would prefer putting this at section 3 because this could justify why using GAN for faster mixing is valid; then we can say mcmc}

% \subsection{analytic}
% \subsubsection{2d data, with Ring, 2 mode Mixture of Gaussian, 6 mode MoG}

% Plot of distributions, table of ESS, graph for training iterations vs. ESS/acc rate and or 1 step autocorrelation; trace plot for the 6 mode case to show chain is jumping between modes

% \subsubsection{Bayes LR}
% table of ess, graph for training iterations vs. New GAN discriminator loss + ESS




% \se{we should compare to\cite{salimans2015markov}}
% \js{It would be nice if we can do the experiments for HVI on MNIST}
